Counter Attack on Byzantine Generals: Parameterized Model Checking of Fault-tolerant Distributed Algorithms

We introduce an automated parameterized verification method for fault-tolerant distributed algorithms (FTDA). FTDAs are parameterized by both the number of processes and the assumed maximum number of Byzantine faulty processes. At the center of our technique is a parametric interval abstraction (PIA) where the interval boundaries are arithmetic expressions over parameters. Using PIA for both data abstraction and a new form of counter abstraction, we reduce the parameterized problem to finite-state model checking. We demonstrate the practical feasibility of our method by verifying several variants of the well-known distributed algorithm by Srikanth and Toueg. Our semi-decision procedures are complemented and motivated by an undecidability proof for FTDA verification which holds even in the absence of interprocess communication. To the best of our knowledge, this is the first paper to achieve parameterized automated verification of Byzantine FTDA.

==> casestudy.tex <==

\nop{
\section{Case study}\label{sec:casestudy}





\begin{algorithm}[t]
%%
\footnotesize
\setlinenosize{\tiny}
\setlinenofont{\tt}
\begin{algorithmic}[1]
\CODE{$i$ if it is correct}
\VAR{}

\STATE $v_i\in \{ \false, \true \}$
\STATE $\accept_i\in\{ \false, \true  \}\leftarrow \false$
\EMPTY

\TRANS{}

\IF{$v_i$ {\bf and} not sent $\echomsg$ before}
\label{alg:init1}
\STATE \emph{send} $\echomsg$ to all;
\ENDIF

\IF{\emph{received} $\echomsg$ from at least $t+1$ \emph{distinct}
  processes\\ \qquad {\bf and} not sent $\echomsg$ before}
\label{alg:tp1}
\STATE \emph{send} $\echomsg$ to all;
\ENDIF

\IF{\emph{received} $\echomsg$ from at least $n-t$ \emph{distinct}
processes}
\label{alg:nmt}
\STATE $\accept_i \leftarrow \true$;\label{alg:end}
\ENDIF

\end{algorithmic}
\caption{ Core logic of the broadcasting algorithm from~\cite{ST87:abc}.}
\label{alg:ST87}
\end{algorithm}


In our case study, we analyze Algorithm~\ref{alg:ST87}, which is a
     simplified version of the broadcasting primitive by Srikanth and
     Toueg~\cite{ST87}.
In this section we first describe the computational model and
     Algorithm~\ref{alg:ST87} from a \emph{distributed algorithms
     point of view}, and will then show how to capture the algorithm
     in our modeling framework.





\paragraph{Computational model for asynchronous distributed
  algorithms}

We recall the standard assumptions for asynchronous distributed
     algorithms. As mentioned in the introduction,
a system consists of $n$ processes out of which at most $t$ may be
     faulty.
When considering a fixed computation, we denote by $f$ the actual
     number of faulty processes.
It is assumed that $n>3t \wedge f \leq t \wedge t>0$.
%% \hv{E.g.
%% here.
%% Reuse terminology + references to above sections}
 Correct processes
     follow the algorithm, in that they take steps that correspond to
     the algorithm description.
Between every pair of processes, there is a bidirectional link over
     which messages are exchanged.
A link contains two message buffers, each being the receive buffer of
     one of the incident processes.

%%\hv{I don't understand what ``models''and ``buffers'' means here exactly}


A step of a correct process is atomic and consists of
     the following three parts.
First a process receives a possibly empty subset of the messages in
     its buffer, then it performs a state transition depending on its
     current state and the received messages.
Finally, a process may send at most one message to each process, that
     is, it puts a message in the buffer of the other processes.

Computations are  asynchronous in that the steps can be arbitrarily
     interleaved, provided that each correct process takes an infinite
     number of steps.
%%\hv{this needs to be related to our discussion about acyclic CFAs etc.}
%%\jw{I do not think that such a discussion fits here, from a
     %%d.a. point of view...}
Moreover, if a message $m$ is put into a process $p$'s buffer, and $p$
     is correct, then $m$ is eventually included in the set of
     messages received.
This property is called \emph{reliable communication}.
Faulty processes are not restricted, except that they have no influence
     of the buffers of links to which they are not incident.
This property is often called \emph{non-masquerading}, as a faulty
     process cannot ``pretend'' to be another process.
 }

\nop{

\input{CFAex.tex}

\paragraph{Specific details of Algorithm~\ref{alg:ST87}}

The code is typical pseudocode found in the distributed algorithms
     literature.
The \codelinerange{alg:init1}{alg:end} describe one step of the
     algorithm.
The receiving is implicit and performed before
     \codelineref{alg:init1}, and the possible sending of messages is
     deferred to the end, and is performed after
     \codelineref{alg:end}.

We observe that a process always sends to all.
Moreover, \codelinerange{alg:init1}{alg:end} only
     consider messages of type $\echomsg$, while all other messages
     are ignored.
Hence, a Byzantine faulty process has an impact on
     correct processes only if they send an $\echomsg$ when they
     should not or vice versa.
Note that faulty processes may behave two-faced, that is, send messages
     only to a subset of the correct processes.
%% \hv{Is ``two-faced'' standard terminology?}
%% \jw{yes, it is the folklore intuition of the worse behavior of
%%   Byzantine faults}
Moreover, faulty processes may send multiple $\echomsg$ messages to a
     correct process.
However, from the code we observe that multiple receptions of such
     messages do not influence the number of messages received by
     ``distinct'' processes due to non-masquerading.
Finally, the condition ``not sent $\echomsg$ before'' guarantees that
     each correct process sends $\echomsg$ at most once.






\paragraph{Our modeling choices}


The most immediate choice is that we consider the set of parameters
     $\paraset$ to be $\{n, t, f\}$ and $RC(n, t, f) = n>3t \wedge f
     \leq t \wedge t>0$.
In the pseudo code, the status of a process is only implicitly
     mentioned.
The relevant information we have to represent in the status variable
     is (i) the initial state (ii) whether a process has already sent
     $\echomsg$ and (iii) whether a process has set $\accept$ to
     $\true$.
Observe that once a process has sent $\echomsg$, its value of $v_i$
     does not interfere anymore with the further state transitions.
Moreover, a process only sets $\accept$ to $\true$ if it has sent a
     message (or is about to do so in the current step).
Hence, we define the set $\PC$ to be $\{\IT,\RI,\SE,\AC\}$, where
     $\PC_0= \{\IT,\RI \}$.
$\IT$ corresponds to the case where initially $v_i=\false$, and $\RI$
     to the case where initially $v_i=\true$.
Further, $\SE$ means that a process has sent an $\echomsg$ message but
     has not set $\accept$ to $\true$ yet, and $\AC$ means that the
     process has set $\accept$ to $\true$.
Having fixed the status values, we can formalize the specifications we
     want to verify.
They are obtained by the broadcasting specification parts called
     \emph{unforgeability}, \emph{correctness}, and \emph{relay}
     introduced in~\cite{ST87:abc}:
 }

\begin{align}
  \tag{U}
 &\ltlG \left(\left[ \forall i.\; \pc_i \ne \RI \right]
     \rightarrow \ltlG
   \left[\forall j.\;  \pc_j \ne \AC
     \right]\right) \label{ST:u}
\\
  \tag{C}
&\ltlG \left(\left[\forall i.\; \pc_i = \RI \right]
      \rightarrow
   \ltlF  \left[ \exists j.\; \pc_j = \AC\right]
   \right) \label{ST:corr}
 \\
\tag{R}
  &\ltlG \left(\left[\exists i.\; \pc_i = \AC \right]
      \rightarrow \ltlF \left[
   \forall j.\; \pc_j = \AC \right] \right)
\label{ST:rel}
\end{align}

\nop{
As the asynchrony of steps is already handled by our parallel
     composition described in Section~\ref{sec:prelim}, it remains to
     describe the semantics of sending and receiving messages in our
     system model.

Let us first focus on messages from and to correct processes.
As we have observed that each correct process sends at most one
     message, and multiple messages from faulty processes have no
     influence, it would be sufficient to represent each buffer by a
     single variable that represents whether a message of a certain
     kind has been put into the buffer.
As we have only $\echomsg$ messages sent by correct processes, it is sufficient 
	 to model one variable per buffer.
Moreover, if we only consider the buffers between correct processes,
     due to the ``send to all'' it is sufficient to capture all
     messages between correct processes in a single variable.
To model this, we introduce the shared variable $\sent$.

The reception of messages can then be modeled by a local variable
     $\rcvd$ whose update depends on the messages sent.
In particular, upon a receive, the variable $\rcvd$ can be increased
     to any value less than or equal to $\sent$.

It remains to model faults.
Remark~\ref{rem:symmetry} makes clear that our system model requires
     us to have identical processes.
This allows at least the two possibilities to model faults:
\begin{itemize}

\item we capture whether a process is correct or faulty as a flag in
     the status, and require that in each run $f\le t$
     processes are faulty.
Then we would have to derive a CFA sub-automaton for faulty processes,
     and would need additional variables to capture sent messages by
     faulty processes.

\item we consider the system to consist of correct processes only,
     let $\syssize(n,t,f) = n-f$, and model only the influence of
     faults, via the messages correct processes may receive.
This can be done by allowing each correct process to receive at most
     $f$ messages more than sent by correct ones, that is that $\rcvd$
     can be increased to any value less than or equal to $\sent + f$.

\end{itemize}

We have chosen the latter approach.
Based on this discussion we directly obtain the CFA given in
     Figure~\ref{Fig:STCFA} that describes the steps of
     Algorithm~\ref{alg:ST87}.
Note that its structure follows the pseudo code description of
     Algorithm~\ref{alg:ST87} very closely.

 }


\paragraph{Verification strategy for liveness}
\label{sec:veriDA}


Relevant liveness properties can typically only be guaranteed if the
     underlying system ensures some fairness guarantees.
In asynchronous distributed systems one assumes for instance
     communication fairness, that is, every message sent is eventually
     received.
The statement $\forall i.\; \rcvd_i \ge \sent_i$ describes a
     global state where all messages are received by processes.
     It follows that a justice constraint $q_{CF} \in \PropVAR$ defined as
$$
q_{CF} = \quotes{\forall i.\; \rcvd_i \ge \sent_i } \tag{CJ} \label{eq:CJ}
$$
 states that the system infinitely often reaches a state where communication
 communication medium delivered all messages.
We only require a liveness specification $\varphi$ to be
     satisfied if the system is communication fair.
     Our approach is to automatically verify $\varphi$ in a
     system under justice constraints $J = \{ q_{CJ}\}$.

\nop{

As (\ref{F:RC}) is a negation-free \ACTL\ formula  over $\PropVAR$,
     and (\ref{ST:corr}) and (\ref{ST:rel}) are  \ACTL\ formulas over
     $\PropPC$, we may verify liveness, that is, (\ref{ST:corr}) and
     (\ref{ST:rel}), based on Corollary~\ref{cor:completeSound}.
For checking safety (\ref{ST:u}) fairness does not have to be treated
     in a special~way.

\smallskip

Note that along all paths where communication is fair, the value of
     $\rcvd_i$ has at least to reach the value of $\sent_i$.
Since $\rcvd_i$ can only increase upon a step by $i$, in some sense,
     $i$ is forced to take steps as long as it has not received
     messages yet.
That is, by this modeling, communication fairness implies some form
     of computation fairness.



%\exclude{
%\input{loop.tex}
%}

\paragraph{Modeling other fault scenarios}

Fault scenarios other than Byzantine faults can be modeled by changing
     the system size, using conditions similar to (\ref{F:RC}), and
     slightly changing the CFA.
More precisely, by changing the non-deterministic assignment (the edge
     leaving $q_I$) that corresponds to receiving messages.
For instance, replacing Byzantine by send omission process
     faults~\cite{NT90} could be modeled as follows: Faulty processes
     could me modeled explicitly by setting $\syssize(n,t,f) = n$.
That at most $f$ processes may fail to send messages, could be modeled
     by $\ctlA \ltlF \ltlG \left[\exists i.\; \rcvd_i + f < \sent_i
     \right]$.
Finally, in this fault model processes may receive all messages sent,
     that is,  $\rcvd :=
     \CFApickOp{\CFAdummy}{\CFApick}{\rcvd\le\CFAdummy  \; \wedge \;
     \CFAdummy \le\sent}$.
By similar adaptations one models, e.g., corrupted communication
     (e.g., due to value faulty links) \cite{SW89}, or hybrid fault
     models \cite{BSW11:hyb} that contain different fault scenarios.

 }



==> simulation.tex <==
\section{Simulation in VASS} 

In this section we give the details of constructing $\VassSymb$ and
$\VassInitSymb$ using a CFA $A=(Q,q_I,q_F,E)$.
 Without loss of generality we assume that $A$ is given in a static single
assignment form (SSA). It means that along every path from $q_I$ to $q_F$ every
variable $x \in \{\pc\} \cup \locset \cup \globset$ is met as a left-hand side
of '$\CFApc := \CFAloc$', '$\CFAinc \; x$', and '$x :=
\CFApickOp{\CFAdummy}{\CFApick}{\CFAcond}$' at most once. One can translate any
CFA into SSA~\cite{Cytron1991} by introducing auxiliary variables that are not
part of the skeleton state.

Given a finite set $X$, we can assign a unique number to each element from $X$,
i.e. give an injective function $ord_X: X \rightarrow \{0,\dots,|X|-1\}$.
Given a status variable $\pc$ and a set of local variables $\locset=\{x_1,
\dots, x_k \}$, we choose an arbitrary order on $\locset$ and construct an
arithmetic expression $idx(\pc, \locset)$ that assigns a unique integer to
every tuple from the set of local states $\localstates = \PC \times
\absdomain^{|\locset|}$:

\begin{align}
idx(sv, \locset) = ord_{\PC}(\pc) + |\PC| \cdot (\Sigma_{i=1}^k |\absdomain|^{i-1} \cdot ord_{\absdomain}(x_i))
\end{align}

For every $e = (q, op, q') \in E$ let $s(e)$ and $t(e)$ denote $q$ and
$q'$ respectively. For every $q \in Q$ by $out(q)$ we denote the set
$\{e \mid s(e) = q \}$. Given a set of variables $X$, by $X'$ we denote
a set of primed variables: $X' = \{x' \mid x \in X \}$.

We further construct $\VassSymb(A)$ as a formula over the variables from $\paraset
\cup \{\pc, \pc'\} \cup \locset \cup \locset' \cup \globset \cup \globset' \cup
\{k, k', \Delta\}$. The variables $k$ and $k'$ are fixed size arrays of
non-negative integers, whose indices range over $\{0, \dots, |\PC| \cdot
|\absdomain|^{|\locset|} - 1\}$. Essentially, the arrays store counters of processes
that reside in a local state corresponding to the array index.  The variable
$\Delta$ is a non-negative integer, keeping the number of processes that make the
same transition.

The $\VassSymb(A)$ is constructed as follows:

\begin{align}
\VassSymb(A) &= \ResCond \wedge compute \wedge dec \wedge inc \wedge counters \\
compute &= pick(q_I) \wedge \Wedge{e \in E}{} \big( on_e \rightarrow pick(t(e)) \big)\label{eq:compute}\\
pick(q) &= \Vee{e \in out(q)}{} \big(on_e
    \wedge \phi_{op}(e) \wedge \Wedge{f \in out(q) \setminus \{e\}}{}
     \neg on_{f}\big) \label{eq:pick} \\
    dec &= (k'(idx(sv, \locset)) = k(idx(sv, \locset)) - \Delta) \label{eq:dec} \\
    inc &= (k'(idx(sv', \locset')) = k(idx(sv', \locset')) + \Delta) \label{eq:inc}\\
counters &= \Wedge{i=0}{|\localstates|-1} \big(k(i) \ge 0 \wedge k'(i) \ge 0\big)
\end{align}

The formula $compute$ describes a simple path through the CFA $A$. Note, that
$A$ is acyclic and all automata states are reachable from $q_I$.
It starts with the initial state $q_I$ and for
each state $q$ on the path exactly one outgoing edge is enabled by the
subformula $pick(q)$.  An edge $e \in E$ is enabled if and only if the
auxiliary variable $on_e$ evaluates to true. The effect of the
operation $op \in Op$ associated with $e$ is encoded by the formula
$\phi_{op}(e)$. The formulae $inc$ and $dec$ encode increment and decrement of
process counters by $\Delta$ for the previous local state ($\{sv\} \cup
\locset$) and the next local state ($\{sv'\} \cup \locset'$) respectively.

The translation of operations is captured by $\phi_{op}$ that is summarized in
the tables~\ref{ref:trans-cond}, \ref{ref:trans-op}. The formula is constructed
similarly to the abstract semantics $\models_{abs}$ given in the
table~\ref{sem:abst}. However, the global variables from $\globset$ are treated
as variables over the concrete domain $D$. This affects the
equations~\ref{eq:le-mixed}, \ref{eq:le-conc-threshold}, and~\ref{eq:increment-abs}.
In the equations~\ref{eq:le-mixed} and \ref{eq:le-conc-threshold} global variables
are compared against threshold expressions over concrete parameters.
The equation~\ref{eq:increment-abs} reflects the fact that $\Delta$ processes perform
the same transition in a single step. Thus, the value of a global variable increments
by $\Delta$ instead of 1.

\begin{table*}
\begin{align}
\phi_{cond}(\squotes{y \le x + e}) & :=
    \Vee{\absSym_i, \absSym_j:\ \absSym_j \in \absPlus{e}(\absSym_i)}{} (y = \absSym_j \wedge x = \absSym_i)
        & \mbox{ when } x, y \in \locset \label{eq:le-abstract} \\
\phi_{cond}(\squotes{y \le x + e}) & :=
    \Vee{\absSym_i, \absSym_j:\ \absSym_j \in \absPlus{e}(\absSym_i)}{} (y = \absSym_j \wedge \thresh_i \le x \le \thresh_{i+1})
        & \mbox{ when } x \in \globset, y \in \locset \label{eq:le-mixed} \\
\phi_{cond}(\squotes{\thresh_i \le x}) & := \Vee{\absSym \le \absSym_i}{} x = \absSym
        & \mbox{ when } x \in \locset \label{eq:le-abs-threshold}\\
\phi_{cond}(\squotes{\thresh_i \le x}) & := \thresh_i \le x
        & \mbox{ when } x \in \globset \label{eq:le-conc-threshold}\\
\phi_{cond}(\squotes{\CFApc = \CFAloc}) & := \CFApc = \CFAloc \label{eq:eq-pc}\\
\phi_{cond}(\squotes{g_1 \wedge g_2}) & := \phi(g_1) \wedge \phi(g_2) \\
\phi_{cond}(\squotes{\neg g_1}) & := \neg (\phi(g_1))
\end{align}
\caption{Translating conditions \texttt{atomcond} and \texttt{guard} of CFA}
\label{ref:trans-cond}
\end{table*}

\begin{table*}
\begin{align}
  \phi_{op}((q, \squotes{\CFAguard}, q')) &
        := \phi_{cond}(\CFAguard) \\
  \phi_{op}((q, \squotes{\CFApc := \CFAloc}, q')) &
        := (\CFApc' = \CFAloc) \\
  \phi_{op}((q, \squotes{\CFAinc \; x}, q')) &
        := \Vee{d, d':\ d' \in \absPlus{1}(d)}{} x = d \wedge x' = d' &
        \mbox{ if } x \in \locset \label{eq:increment-conc} \\
  \phi_{op}((q, \squotes{\CFAinc \; x}, q')) &
        := (x' = x + \Delta) &
        \mbox{ if } x \in \globset \label{eq:increment-abs} \\
  \phi_{op}((q, \squotes{x := \CFApickOp{\CFAdummy}{\CFApick}{\CFAcond}}, q')) &
        := (\phi_{cond}(\CFAcond[x'/\CFAdummy]))
\end{align}
\caption{Translating edges $e \in E$ of CFA}
\label{ref:trans-op}
\end{table*}


\begin{proposition}
For every CFA $A$ and for all $\param \in \paraset$ if in a system instance
$\ConcSys = (S_I,S^0_I, R_I, AP, \labelfun_I)$ a process makes a transition
$(s, s') \in R$ resulting in a system transition $(\gst, \gst') \in R_I$,
then $\VassSymb$ is satisfiable with the following
constraints on variables:
\begin{align}
    \mbox{ It holds } & sv = s.sv \mbox{ and } sv' = s'.sv \\
    \mbox{For every } x \in \locset \mbox{ it holds }
        & x = \absMap(s.x) \mbox{ and } x' = \absMap(s'.x) \\
    \mbox{For every } y \in \globset \mbox{ it holds }
        & y = \sigma.y \mbox{ and } y' = \sigma'.y \\
    \mbox{For every } \ell \in \localstates \mbox{ it holds }
        & k(idx(\ell)) = K(\absMapSys(\sigma), \ell) \\
    \mbox{ and } & k'(idx(\ell)) = K(\absMapSys(\sigma'), \ell) \\
    &\Delta = 1 
\end{align}
\end{proposition}

Thus $\VassSymb(A)$ simulates every $\ConcSys$.

\begin{proposition}
For every CFA $A$, for any set of variables satisfying $\VassSymb$
there is a transition $(w, w') \in R_\CntASys$ satisfying the following constraints:
\begin{align}
    & \param = (p_1, \dots, p_{|\paraset|})\\
    \mbox{For every } \ell \in \localstates \mbox{ it holds }
        & w.\absCnt{\ell} = \afunc{\param}{k(idx(\ell))} \\
    \mbox{ and }
        & w'.\absCnt{\ell} = \afunc{\param}{k'(idx(\ell))} \\
    \mbox{For every } x \in \globset \mbox{ it holds }
        & w.y = \afunc{\param}{y} \mbox{ and } w'.y = \afunc{\param}{y'} \\
\end{align}
\end{proposition}

\textbf{TODO}: $\VassInitSymb$...
\textbf{TODO}: Give the invariant in terms of $\VassSymb$...
\textbf{TODO}: Say smth about completeness...


==> table-incorrect.tex <==
\setcounter{rowno}{0}
  \begin{tabular}{|rrrrrrrr|}
   \hline
   \textbf{\scriptsize{$M \models \varphi$}} & \textbf{\scriptsize{RC}} & \textbf{\scriptsize{Spin}} & \textbf{\scriptsize{Spin}} & \textbf{\scriptsize{Spin}} & \textbf{\scriptsize{Spin}} & \textbf{\scriptsize{Ref-t}} & \textbf{\scriptsize{Total}} \\
    & & \textbf{\scriptsize{Time}} & \textbf{\scriptsize{Memory}} & \textbf{\scriptsize{States}} & \textbf{\scriptsize{Depth}} & \textbf{\scriptsize{Steps}} & \textbf{\scriptsize{Time}} \\
   \hline
Byz $\not \models$ U & (a) & 7.15 s & 168 MB & 3160k & 23120 & 12 & 85 s\\
Byz $\not \models$ C & (a) & 3.21 s & 100 MB & 1123k & 17829 & 6 & 28 s\\
Byz $\not \models$ R & (a) & 0.43 s & 71 MB & 136k & 6387 & 9 & 23 s\\
B $\models$ U & (b)& 3.96 s & 103 MB & 1192k & 11073 & 0 & 5 s\\
B $\models$ C &  (b) & 8.95 s & 175 MB & 3781k & 36757 & 19 & 104 s\\
B $\not \models$ R & (b) & 2.99 s & 110 MB & 1451k & 24656 & 43 & 165 s\\
Sym $\not \models$ U & (a) & 0.09 s & 68 MB & 31k & 1503 & 1 & 1 s\\
S $\not \models$ C & (a) & 0.08 s & 68 MB & 32k & 1837 & 3 & 3 s\\
S $\models$ R & (a) & 0.17 s & 69 MB & 54k & 2161 & 6 & 16 s\\
O $\models$ U & (c) & 0.03 s & 68 MB & 6k &544 & 0 & 1 s\\
O $\not \models$ C & (c) & 0.03 s & 68 MB & 6k & 544 & 0 & 2 s\\
O $\not \models$ R & (c) & 0.01 s & 68 MB & 0.1k & 481 & 0 & 4 s\\
   \hline
  \end{tabular}
     \caption{Experimental data on abstraction
     of fault-tolerant algorithms with incorrect resilience conditions (RC):
        (a) $f \le t +1$; (b) $n \ge 3t$; (c) $n \ge 2t$.}
\label{tab:inC}


==> technical_challenge.tex <==

%\paragraph{Technical Challenges and Related Work.}

